Supervised Feature Subset Selection and Feature Ranking for Multivariate Time Series without Feature Extraction

We introduce supervised feature ranking and feature subset selection algorithms for multivariate time series (MTS) classification. Unlike most existing supervised/unsupervised feature selection algorithms for MTS our techniques do not require a feature extraction step to generate a one-dimensional feature vector from the time series. Instead it is based on directly computing similarity between individual time series and assessing how well the resulting cluster structure matches the labels. The techniques are amenable to heterogeneous MTS data, where the time series measurements may have different sampling resolutions, and to multi-modal data.

==> 02related_works.tex <==
\section{Related Works}
\label{sec:related_work}
\noindent\textbf{Feature Selection of Multivariate Time Series.} Feature subset selection~\cite{yoon2005feature}.





==> obsolete.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse%commet out the feature matrix story
\subsubsection{Verify the Correctness}
To evaluate the correctness and effectiveness of our proposed method, we compare our algorithm with existing famous feature selection algorithms, they are:
\begin{itemize}
    \item [1.] \textit{Fisher Score}~\cite{peh2007ro}.
    \item [2.] \textit{mRMR}~\cite{peng2005feature}.
    \item [3.] \textit{ReliefF}~\cite{robnik2003theoretical}.
    \item [4.] \textit{RFS}~\cite{nie2010efficient}.
\end{itemize}

\begin{figure}[h!]
    \centering
    \begin{minipage}[c]{\columnwidth}
    \centering
    \includegraphics[width=0.45\textwidth]{FIG/lymphoma_nmi.pdf}
    \includegraphics[width=0.45\textwidth]{FIG/lymphoma_acc.pdf}
    \caption*{Lymphoma}
    \end{minipage}
    \begin{minipage}[c]{\columnwidth}
    \centering
    \includegraphics[width=0.45\textwidth]{FIG/carcinom_nmi.pdf}
    \includegraphics[width=0.45\textwidth]{FIG/carcinom_acc.pdf}
    \caption*{Carcinom}
    \end{minipage}
    \begin{minipage}[c]{\columnwidth}
    \centering
    \includegraphics[width=0.45\textwidth]{FIG/lung_nmi.pdf}
    \includegraphics[width=0.45\textwidth]{FIG/lung_acc.pdf}
    \caption*{Lung}
    \end{minipage} 
    \begin{minipage}[c]{\columnwidth}
    \centering
    \includegraphics[width=0.45\textwidth]{FIG/yale_nmi.pdf}
    \includegraphics[width=0.45\textwidth]{FIG/yale_acc.pdf}
    \caption*{Yale}
    \end{minipage}
    \begin{minipage}[c]{\columnwidth}
    \centering
    \includegraphics[width=0.45\textwidth]{FIG/orl_nmi.pdf}
    \includegraphics[width=0.45\textwidth]{FIG/orl_acc.pdf}
    \caption*{ORL}
    \end{minipage}
\caption{Experiment results on regular feature matrix data.}
\label{fig:fea_ranking_nmi_acc}
\end{figure}%

\subsubsection{Datesets}
\label{subsec:data}
We select five benchmark datasets that frequent appears in feature selection research works.
\begin{table}[h]
    \centering
    \begin{tabular}{|*{4}{c|}}
    \toprule
        Name & Samples & Feature & Class  \\ \midrule
        Lymphoma & 96 & 4026 & 9 \\
        Carcinom & 174 & 9182 & 11 \\
        Lung & 203 & 3312 & 5 \\
        Yale & 165 & 1024 & 15  \\
        ORL & 400 & 1024 & 40 \\ \bottomrule
    \end{tabular}
    \caption{Description of classical datasets which in the format of feature matrix.}
    \label{tab:data_c}
\end{table}

\subsubsection{Discussion} TBD. The experiment result is show in Fig.~\eqref{fig:fea_ranking_nmi_acc}.

\fi%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




\subsection{Spectral Embedding of Graphs.} The PIE is one of the spectral embeddings for graph. There exists other different spectral embeddings that can be differentiated by the number of vectors ($k$) be used. For example, PIE is the case of $k=1$.
\subsubsection{Spectral Clustering Embedding: $1<k<n$.}
The spectral clustering embedding is the $k$ smallest eigenvectors of normalized random-walk Laplacian matrix $\bm{L}$, which is defined as $\bm{L} = \bm{I} - \bm{D}^{-1}\bm{W}$. Generally, these $k$ smallest eigenvectors define a subspace where the clusters of graph are well separated. For each vertex in the graph $\bm{W}$, the spectral clustering embedding generate a $\mathcal{R}^k$ embedding vector for it.

\subsubsection{Heat Kernel Embedding: $k=n$.} For each vector $u$ in graph $\bm{W}$, the heat kernel embedding $\psi_t(u): V\rightarrow \mathcal{R}^n$ of it is defined as follows:
\begin{equation}
    \psi_t(u) \triangleq \frac{1}{\sqrt{d_u}}\left( e^{-(t/2)\dot \lambda_1}f_1(u), \cdots, e^{-(t/2)\dot \lambda_n}f_n(u) \right),
\end{equation}
where $t \geq 0$ is a fixed constant specified by the user, $d_u$ is the degree of node $u$, $\lambda_i$ and $f_i(u)$ are the eigenvalue and eigenvector of normalized Laplacian matrix $\bm{L}$ respectively.     

